Covariance Matrix Estimation under Total Positivity for Portfolio Selection

Selecting the optimal Markowitz porfolio depends on estimating the covariance matrix of the returns of $N$ assets from $T$ periods of historical data. Problematically, $N$ is typically of the same order as $T$, which makes the sample covariance matrix estimator perform poorly, both empirically and theoretically. While various other general purpose covariance matrix estimators have been introduced in the financial economics and statistics literature for dealing with the high dimensionality of this problem, we here propose an estimator that exploits the fact that assets are typically positively dependent. This is achieved by imposing that the joint distribution of returns be multivariate totally positive of order 2 ($\text{MTP}_2$). This constraint on the covariance matrix not only enforces positive dependence among the assets, but also regularizes the covariance matrix, leading to desirable statistical properties such as sparsity. Based on stock-market data spanning over thirty years, we show that estimating the covariance matrix under $\text{MTP}_2$ outperforms previous state-of-the-art methods including shrinkage estimators and factor models.

==> ir_table.tex <==
% \begin{table}[htb!] \label{table:IR}
% \centering
% \begin{tabular}{l | l | llll}
% \toprule 
% \toprule 
% \makecell{N \\ (nr.~of assets)} & \makecell{T \\ (lookback period)}   & EW-TQ & \makecell{Linear \\ Shrinkage} & \makecell{Approximate \\ Factor Model} &     $\text{MTP}_2$ \\
% \midrule
% 100 & 25   &  0.694 &            0.710 &                    0.730 &    \textcolor{blue}{0.803} \\
%     & 50   &  0.694 &            0.625 &                    0.637 &    \textcolor{blue}{0.849} \\
%     & 100  &  0.694 &            0.600 &                    0.617 &  \textcolor{blue}{0.896**} \\
%     & 200  &  0.694 &            0.670 &                    0.688 &   \textcolor{blue}{0.899*} \\
%     & 400  &  0.694 &            0.736 &                    0.782 &    \textcolor{blue}{0.892} \\
%     & 1260 &  0.694 &            0.831 &                    0.834 &    \textcolor{blue}{0.890} \\
% \midrule
% 200 & 50   &  0.757 &            0.742 &                    0.726 &    \textcolor{blue}{0.853} \\
%     & 100  &  0.757 &            0.719 &                    0.716 &    \textcolor{blue}{0.829} \\
%     & 200  &  0.757 &            0.812 &                    0.800 &    \textcolor{blue}{0.885} \\
%     & 400  &  0.757 &            0.864 &                    0.870 &    \textcolor{blue}{0.886} \\
%     & 800  &  0.757 &            0.967 &                    0.961 &    \textcolor{blue}{0.970} \\
%     & 1260 &  0.757 &            0.906 &                    0.916 &    \textcolor{blue}{0.955} \\
% \midrule
% 500 & 125  &  0.764 &            0.876 &                    0.872 &    \textcolor{blue}{1.019} \\
%     & 250  &  0.764 &            0.985 &                    0.977 &    \textcolor{blue}{1.112} \\
%     & 500  &  0.764 &            0.940 &                    0.980 &    \textcolor{blue}{1.045} \\
%     & 1000 &  0.764 &            0.918 &                    0.978 &    \textcolor{blue}{1.061} \\
% \bottomrule
% \end{tabular}
% \caption{Performance of different estimators for various $N$ (number of assets) and $T$ (number of samples considered). For each combination of $N, T$ and choice of estimator, the number in the table is the information ratio (ratio of the average return to the standard deviation of returns) of the portfolio given by applying the estimator to the rolling out of sample.}
% \end{table}

\begin{table}[b!]
\centering
\begin{tabular}{cc|ccccccc}
\toprule
N    & T     &  EQ-TW &     LS &    NLS &                   AFM- & AFM- & POET & POET \\
 &  &        &        &        &   LS                       &    NLS     &  (k=3)          &    (k=5)        \\
\midrule
100 & 50   &  0.694 &  0.625 &  0.648 &                    0.617 &   0.621 &      0.760 &      0.791 \\
    & 100  &  0.694 &  0.600 &  0.682 &                    0.628 &   0.620 &      0.797 &      0.690 \\
    & 200  &  0.694 &  0.670 &  0.720 &                    0.691 &   0.675 &      0.802 &      0.706 \\
    & 400  &  0.694 &  0.736 &  0.772 &                    0.803 &   0.776 &      0.824 &      0.753 \\
    & 1260 &  0.694 &  0.831 &  0.834 &                    0.832 &   0.831 &      0.841 &      0.831 \\
200 & 100  &  0.757 &  0.719 &  0.735 &                    0.715 &   0.728 &      0.766 &      0.762 \\
    & 200  &  0.757 &  0.812 &  0.793 &                    0.796 &   0.790 &      0.747 &      0.764 \\
    & 400  &  0.757 &  0.864 &  0.885 &                    0.888 &   0.892 &      0.825 &      0.820 \\
    & 800  &  0.757 &  0.967 &  0.961 &                    0.962 &   0.967 &      0.747 &      0.870 \\
    & 1260 &  0.757 &  0.906 &  0.907 &                    0.913 &   0.906 &      0.773 &      0.770 \\
500 & 250  &  0.764 &  0.985 &  0.995 &                    0.997 &   0.993 &      0.869 &      1.030 \\
    & 500  &  0.764 &  0.940 &  0.955 &                    0.995 &   1.003 &      0.849 &      1.027 \\
    & 1000 &  0.764 &  0.918 &  0.976 &                    0.993 &   0.980 &      0.772 &      0.861 \\
    & 1260 &  0.764 &  0.920 &  0.967 &  0.984 &   0.982 &      0.806 &      0.909 \\
\bottomrule
\end{tabular}

\bigskip

%old one
% \begin{tabular}{ccccc}
% \toprule
%  N   &  T    &                     MTP2 &                   GLASSO &                    CLIME \\
%  &  &                          &                          &                          \\
% \midrule
% 100 & 50   &                    0.849 &  \textcolor{blue}{0.858} &                      nan \\
%     & 100  &  \textcolor{blue}{0.896} &                    0.885 &                      nan \\
%     & 200  &  \textcolor{blue}{0.899} &                    0.855 &                    0.830 \\
%     & 400  &  \textcolor{blue}{0.892} &                    0.877 &                    0.852 \\
%     & 1260 &  \textcolor{blue}{0.890} &                    0.878 &                    0.778 \\
% 200 & 100  &                    0.829 &  \textcolor{blue}{0.887} &                      nan \\
%     & 200  &  \textcolor{blue}{0.885} &                    0.859 &                      nan \\
%     & 400  &                    0.886 &                    0.865 &  \textcolor{blue}{0.916} \\
%     & 800  &  \textcolor{blue}{0.970} &                    0.862 &                    0.860 \\
%     & 1260 &  \textcolor{blue}{0.955} &                    0.887 &                    0.845 \\
% 500 & 250  &  \textcolor{blue}{1.112} &                    0.908 &                      nan \\
%     & 500  &  \textcolor{blue}{1.045} &                    0.887 &                      nan \\
%     & 1000 &  \textcolor{blue}{1.061} &                    0.897 &                    0.828 \\
%     & 1260 &  \textcolor{blue}{1.034} &                    0.896 &                    0.858 \\
% \bottomrule
% \end{tabular}


\begin{tabular}{cc|ccccc}
\toprule
 N   &  T    &                        GLASSO &   CLIME & CLIME-&MTP2 & MTP2- \\
 &  &                           &       & KT &     & KT    \\
 
 \midrule
    100 & 50   &                      0.858 &                      nan & 0.788&0.849 &  \textcolor{blue}{0.905}  \\
    & 100  &                      0.885 &                      nan & 0.837&0.896 & \textcolor{blue}{0.975}   \\
    & 200  &                      0.855 &                    0.830 & 0.882&0.899 &  \textcolor{blue}{0.950}  \\
    & 400  &                      0.877 &                    0.852 &  0.823&0.892 & \textcolor{blue}{0.924}  \\
    & 1260 &                      0.878 &                    0.778 & 0.767&\textcolor{blue}{0.890} &  0.855 \\
200 & 100  &                      0.887 &                      nan & 0.844&0.829 & \textcolor{blue}{0.918}   \\
    & 200  &                       0.859 &                      nan & 0.896&0.885&  \textcolor{blue}{0.919} \\
    & 400  &                                        0.865 &  \textcolor{blue}{0.916} & 0.821&0.886 &  0.893  \\
    & 800  &                      0.862 &                    0.860 & 0.805&\textcolor{blue}{0.970} &  0.945 \\
    & 1260 &                      0.887 &                    0.845 & 0.885&\textcolor{blue}{0.955} &  0.931  \\
500 & 250  &                      0.908 &                      nan &  0.596&1.112 & \textcolor{blue}{1.133}  \\
    & 500  &                      0.887 &                      nan & 0.511 &\textcolor{blue}{1.045} & 1.005 \\
    & 1000 &                      0.897 &                    0.828 &  \textcolor{blue}{1.101}&1.061 & 0.993 \\
    & 1260 &                      0.896 &                    0.858 & 0.806 &\textcolor{blue}{1.034} & 0.958 \\
\bottomrule
\end{tabular}\qquad\qquad\;
%\vspace{-0.2cm}
\caption{For each combination of $N$ (portfolio size), $T$ (lookback period), and covariance matrix estimator, we report the out-of-sample information ratio (ratio of the average return to the standard deviation of return) of the portfolio.  The most competitive value in each row is highlighted in blue.
%Performance of different estimators for various $N$ (number of assets) and $T$ (number of samples considered). For each combination of $N, T$ and choice of estimator, the number in the table is the information ratio (ratio of the average return to the standard deviation of returns) of the portfolio given by applying the estimator to the rolling out of sample.
} \label{table:IR}
\end{table}

\begin{comment}
\begin{tabular}{cc|ccccc}
\toprule
 N   &  T    &                      MTP2 &  GLASSO &   CLIME && MTP2- & CLIME-\\
 &  &                           &       &  &     & KT & KT    \\
 
 \midrule
100 & 50   &                    0.849 &  \textcolor{blue}{0.858} &                      nan &&  0.905 & 0.788 \\
    & 100  &  \textcolor{blue}{0.896} &                    0.885 &                      nan && 0.975 & 0.837  \\
    & 200  &  \textcolor{blue}{0.899} &                    0.855 &                    0.830 &&  0.950 & 0.882 \\
    & 400  &  \textcolor{blue}{0.892} &                    0.877 &                    0.852 && 0.924 &  0.823 \\
    & 1260 &  \textcolor{blue}{0.890} &                    0.878 &                    0.778 &&  0.855 & 0.767\\
200 & 100  &                    0.829 &  \textcolor{blue}{0.887} &                      nan && 0.918 & 0.844  \\
    & 200  &  \textcolor{blue}{0.885} &                    0.859 &                      nan &&  0.919 & 0.896\\
    & 400  &                    0.886 &                    0.865 &  \textcolor{blue}{0.916} &&  0.893 & 0.821 \\
    & 800  &  \textcolor{blue}{0.970} &                    0.862 &                    0.860 &&  0.945 & 0.805\\
    & 1260 &  \textcolor{blue}{0.955} &                    0.887 &                    0.845 &&  0.931 & 0.885 \\
500 & 250  &  \textcolor{blue}{1.112} &                    0.908 &                      nan && 1.133 &  0.596 \\
    & 500  &  \textcolor{blue}{1.045} &                    0.887 &                      nan && 1.005 & 0.511\\
    & 1000 &  \textcolor{blue}{1.061} &                    0.897 &                    0.828 && 0.993 &  1.101\\
    & 1260 &  \textcolor{blue}{1.034} &                    0.896 &                    0.858 && 0.958 & 0.806\\
\bottomrule
\end{tabular}
\end{comment}

==> preambule.tex <==
\setlength{\parskip}{1ex plus 0.3ex minus 0.2ex}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\topmargin}{-.5in}
\setlength{\textheight}{8.9in}
\setlength{\oddsidemargin}{0.25in}
\setlength{\evensidemargin}{0.25in}
\setlength{\textwidth}{6.125in}
%\renewcommand{\baselinestretch}{1.1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%`

%\usepackage{refcheck}
\usepackage{graphicx,mathrsfs,epstopdf}
\usepackage{amsmath,amsfonts,amssymb,amsthm}
\usepackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\usepackage{algorithm} % has to be loaded AFTER hypperrf
\usepackage{algorithmicx}
\usepackage{algpseudocode}
\usepackage{framed} % for highlighting paragraph
\usepackage{blkarray}

%\usepackage{natbib}
\usepackage{enumerate}
\usepackage{subfigure}
\usepackage{tikz}
\usetikzlibrary{chains,matrix,scopes,fit,decorations,positioning,shapes,snakes,arrows,decorations.markings}
\DeclareGraphicsRule{.tif}{png}{.png}{`convert #1 `dirname #1`/`basename #1 .tif`.png}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%theorems etc.
\newtheorem{thm}{Theorem}[section]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}

\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\newtheorem{const}[thm]{Construction}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{ex}[thm]{Example}
\newtheorem{assp}[thm]{Assumption}

\theoremstyle{remark}
\newtheorem{rem}[thm]{Remark}
\newtheorem{note}{Note}
\newtheorem{ques}{Question}

%operators


\DeclareMathOperator{\rk}{rk} 
\DeclareMathOperator{\cl}{cl}
\DeclareMathOperator{\Supp}{supp}
\DeclareMathOperator{\Sec}{Sec}
\DeclareMathOperator{\tr}{tr} 


%other commands

\newcommand\fr[1]{\lfloor{#1}\rfloor}
\newcommand\frup[1]{\lceil{#1}\rceil}
\newcommand\map{\dasharrow}
\newcommand\la{\lambda}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\A}{\mathbb{A}}
\newcommand{\cO}{\mathcal{O}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\renewcommand{\S}{\mathbb{S}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\RLCT}{{\rm RLCT}}
%\newcommand{\indep}{{\;\bot\!\!\!\!\!\!\bot\;}}
\newcommand{\indic}{{1\!\!1}}
\newcommand{\nmapsto}{{\;\mapsto\!\!\!\!\!\!\!\slash\;}}
\newcommand{\bs}{\boldsymbol}
\newcommand{\mtp}{{\rm MTP}_{2}}
\newcommand{\mwst}{{\rm MWST}}
\newcommand{\tp}{{\rm TP}_{2}}
\newcommand{\cov}{{\rm cov}}
\newcommand{\cd}{\,|\,}
\newcommand{\cip}{\mbox{\,$\perp\!\!\!\perp$\,}}
\newcommand{\indep}{\cip}
\newcommand{\gse}{\,\mbox{$\perp_{G}$}\,}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\proofname{\indent {\sl Proof.}}
\newcommand{\piotr}[1]{{\color{red} \sf $\clubsuit$ Piotr: #1}}
\newcommand{\steffen}[1]{{\color{blue} \sf $\heartsuit$ Steffen: #1}}
\newcommand{\caroline}[1]{{\color{green} \sf $\clubsuit$ Caroline: #1}}

 \newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
    \def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand\notindependent{\!\perp\!\!\!\!\not\perp\!}
\newcommand{\tl}{\triangleleft}
\newcommand{\pto}{{\mathcal{P}_2}}
\newcommand{\spa}{\mathcal{X}}



==> random.tex <==
% @article{bickel2004,
% author = "Bickel, P. and Levina, E.",
% journal = "Bernoulli",
% pages = "989--1010",
% volume = "10",
% year = "2004"
% }
